Clinically-Inspired Multi-Agent Transformers for Disease Trajectory Forecasting from Multimodal Data

Deep neural networks are often applied to medical images to automate the problem of medical diagnosis. However, a more clinically relevant question that practitioners usually face is how to predict the future trajectory of a disease. Current methods for prognosis or disease trajectory forecasting often require domain knowledge and are complicated to apply. In this paper, we formulate the prognosis prediction problem as a one-to-many prediction problem. Inspired by a clinical decision-making process with two agents -- a radiologist and a general practitioner -- we predict prognosis with two transformer-based components that share information with each other. The first transformer in this framework aims to analyze the imaging data, and the second one leverages its internal states as inputs, also fusing them with auxiliary clinical data. The temporal nature of the problem is modeled within the transformer states, allowing us to treat the forecasting problem as a multi-task classification, for which we propose a novel loss. We show the effectiveness of our approach in predicting the development of structural knee osteoarthritis changes and forecasting Alzheimer's disease clinical status directly from raw multi-modal data. The proposed method outperforms multiple state-of-the-art baselines with respect to performance and calibration, both of which are needed for real-world applications. An open-source implementation of our method is made publicly available at \url{https://github.com/Oulu-IMEDS/CLIMATv2}.

==> _responses.tex <==
\onecolumn
\overview{Response Letter to Reviewers}
\newperson{Reviewer 1}{R1}

\question{This work aims to perform disease prognosis forecasting with multimodal data. The current issues in this problem are mainly caused by the required domain knowledge. There are two transformer-based components in the proposed framework, in which one is for analyzing image data, and the other for processing the clinical data. The temporal information is captured by the transformer states. The effectiveness of the proposed approach is validated on predicting the development of structural knee osteoarthritis and Alzheimer’s disease. The performance of the proposed method also outperforms the previous state-of-the-art baselines.
This paper is well organized, well-written, and the motivation is clear.}

\answer{We appreciate the reviewer’s feedback and the provided insightful comments, which we addressed below in a point-to-point manner.}

\question{The proposed concept shown in Fig. 1 is interesting and novel, in which the radiologist is modeled by a transformer block. However, I am concerned that if it is raliable to model the radiologist by a learnable model? As the model is always trained from scratch, the training may be unstable at the beginning and lead to worse convergence. So, if any prior knowledge is needed for this radiologist block?}

\answer{Thanks for your comment that helps us to clarify the training process. In all our experiments, we made use of pre-trained weights of ResNet18 and 3D-ShuffleNet2 for the KOA and AD data, respectively. We improved the clarity of the Implementation details section by supplementing the information at lines~\ref{ln:exp_pretrained_resnet} and~\ref{ln:exp_pretrained_3dshufflenet}. For the reviewer's concern about the convergence, we conducted an ablation study to compare the following three settings: 
\begin{enumerate}
    \item Scratch: We trained the whole framework from scratch. 
    \item Pre-trained two-stage: We utilized the pre-trained weights of ResNet18 for the imaging feature extractors. In the first stage, we merely trained the network on the KL grading in 50 epochs. In the second stage, we trained the whole network on the KL forecasting task in 50 epochs.
    \item Pre-trained end-to-end: We trained the whole network on the KL forecasting task with ResNet18 pre-trained weights. 
\end{enumerate}
In Fig. 1 below, we observed no substantial differences among those settings. In the first and third settings, the convergence was substantially fast, which happened around 20 epochs.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/Ablation_studies/ablation_training.pdf}
    \caption{Ablation study on training strategies. We reported the validation performances over the first 4-year targets on the KL forecasting task.}
    % \label{fig:my_label}
\end{figure}} 

% \todo[inline]{I think that what reviewer is asking, is an experiment. Train the radiologist-like module first, and then start from this initialization instead of training the whole thing from scratch. Another experiment, which would make the rebuttal strong, would be the following: train the radiologist network, freeze the module, and train the GP module ONLY. Then train the whole thing.}

\question{Compared with CLIMATv1, there is a consistency loss added in CLIMATv2. I can get that such consistency regularization will help reserve the features learned from the image domain. However, if this consistency loss will be harmful for the model learning from the contextual clinical information? }

\answer{We understand your concern about the consistency regularization. Therefore, the very first experiment we performed is to evaluate how the regularizer affects other hyperparameters of the framework. As demonstrated in~\cref{tbl:hyperparam_selection}, the value of $\lambda$ associated with the consistency regularization should be $0.5$, which indicates that it contributes to the improvement of the model, but its contribution should be less than the primary loss $\mathcal{L}_{\mathrm{prog}}$.
% The intution of the consistency constraint is to enforce the mutual interaction between the two agents. While the radiologist uses only imaging data, the general practitioner takes into account multimodalities.
}

\question{The data used in the experiments is effective. However, if the p-value can be further reported to validate the effectiveness of the models?}

\answer{Thank to the reviewer for the suggestion. We conducted Wilcoxon signed-rank tests~\cite{wilcoxon1992individual} to compare CLIMATv2 to each baseline on the disease trajectory forecasting task. As such, we described the statistical tests at Line~\ref{ln:wilcoxon_test_desc}, and enhanced~\cref{fig:oai_performances} and~\cref{tbl:adni_performances} with statistical indicators for significant differences. Specifically, we used pairs of p-value thresholds of ($0.0025,0.0005$) and ($0.05, 0.001$) for the experiments on the OAI and ADNI datasets, respectively. The p-value thresholds corresponding to the knee data were adjusted because we performed the evaluation on both knees.}

% \todo[inline]{Comment from Matthew: It's not immediately clear to me what * vs ** means.  I am writing this comment after reading the response and looking at Fig 6 and Tab V - maybe you describe in the text.  Is it for the two p-value thresholds?  Which one corresponds with which?}

\question{In Table III, the new CLIMATv2 slightly outperforms CLIMATv1 under year1 setting, no performance gain under year2 setting, and even performance drop under year4 setting, which looks wired. Such phenomenon can also be observed in Fig. 6 (e) and (g). Could you please give more explanations on this? If it is caused by the ruined clinical feature as mentioned in Q2? }

\answer{As an upgrade of CLIMATv1, the second version of CLIMAT placed emphasis on both performance and calibration. As stated in the second contribution of this study at Line~\ref{ln:2nd_contribution}, our objective was to maintain its performance while achieving better calibration in comparison with the prior version. The literature suggests that the complexity and performance of deep learning models tend to be inversely proportional to their calibration (e.g., measured by expected calibration error (ECE)), especially when the optimization employed the cross-entropy loss as pointed out in~\cite{guo2017calibration,ghosh2022adafocal}. As shown in Table III (now referenced as \cref{tbl:adni_performances}) and Figure~\ref{fig:oai_performances} (e,g), while the differences in performance between the two versions of CLIMAT are mostly insignificant (e.g., there are performance overlappings due to standard errors over multiple runs), the second version consistently achieves substantial lower ECEs compared to its predecessor on most of the tasks. We clarified the advantage of CLIMATv2 compared to CLIMATv1 at Line \ref{ln:conclusion_optimization} in~\cref{sc:conclusions}.}
% \todo[inline]{You need to refer to text when you say that our objective was....}
% \todo[inline]{You can also refer to literature suggesting that calibration and accuracy are hard to improve together}
% \todo[inline]{Make sure that you have something about performance drop in the discussion. Refer to those lines.}

\question{The authors try to give the heatmaps of some cases to show the interpretability of the model, but the result in Fig. 8 (a) is not good at all. The attention areas are located on the borders of the image. Could you elaborate more successful cases as well as failure ones?}

\answer{Previously, we generated the heatmap in~\cref{fig:adni_img_interpretability} by applying max-pooling over multiple self-attention heads, which resulted in noisy highlighted regions as pointed out by~\cite{nirthika2022pooling}. Following~\cite{nirthika2022pooling}, we utilized average pooling instead of max-pooling. We updated~\cref{fig:adni_interpretability} accordingly. This improved the results based on our observarions, but there were still some failure cases. Therefore, as suggested by the reviewer, we presented both successful and unsuccessful cases in~\cref{fig:adni_attn_examples}, and introduced a discussion on this topic. Specifically, the limitation of our framework is mentioned at Line~\ref{ln:attn_limitation} in~\cref{sc:conclusions}. We further emphasize that the naive use of attention might result in unexplainable behaviors as seen in other papers, e.g. Figure 5 in [5], Figure 6 in [6], and Figures 10, 11, and 12 in [7].
\begin{itemize}
    \item[] [4] R. Nirthika, S. Manivannan, A. Ramanan, and R. Wang, “Pooling in convolutional neural networks for medical image analysis: a survey and an empirical study,” Neural Computing and Applications, vol. 34, no. 7, 764 pp. 5321–5347, 2022.  
    \item[] [5] Rao, Yongming, et al. "Counterfactual attention learning for fine-grained visual categorization and re-identification." Proceedings of the IEEE/CVF International Conference on Computer Vision. 2021.
    \item[] [6] Petit, Olivier, et al. "U-net transformer: Self and cross attention for medical image segmentation." Machine Learning in Medical Imaging: 12th International Workshop, MLMI 2021, Held in Conjunction with MICCAI 2021, Strasbourg, France, September 27, 2021, Proceedings 12. Springer International Publishing, 2021.
    \item[] [7] Odusami, Modupe, Rytis Maskeliūnas, and Robertas Damaševičius. "An intelligent system for early recognition of Alzheimer’s disease using neuroimaging." Sensors 22.3 (2022): 740.
\end{itemize}}
% \todo[inline]{This does not feel justified at all. It feels like cherry-picking. The reviewer wants you to discuss WHY you may have good heatmaps and bad heatmaps. The discussion needs to provide a very plausible explanation.}
\question{As the current comparison methods are too naïve and old, if there are any possible newer ones, such as [1] (also based on both image and contextual data)?
\begin{itemize}
    \item[] [1] Wang, Zhiqin, et al. "GPDBN: deep bilinear network integrating both genomic data and pathological images for breast cancer prognosis prediction." Bioinformatics 37.18 (2021): 2963-2970.
\end{itemize}}

\answer{Thanks for your suggestion regarding including new baselines. We compared our methods to 3 more transformer-based baselines: Reformer [1], Informer [2], and Autoformer [3]. The last 2 references were suggested by review 2. We provided the new baselines' results~\cref{fig:oai_performances} and~\cref{tbl:adni_performances}, and presented them at Line~\ref{ln:exp_oai_former_results} in~\cref{sc:perf_comparisons}.
\begin{itemize}
    \item[] [1] Zhou, Haoyi, et al. "Informer: Beyond efficient transformer for long sequence time-series forecasting." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 35. No. 12. 2021.
    \item[] [2] Wu, Haixu, et al. "Autoformer: Decomposition transformers with auto-correlation for long-term series forecasting." Advances in Neural Information Processing Systems 34 (2021): 22419-22430.
    \item[] [3] Kitaev. N. et al. "Reformer: The Efficient Transformer." International Conference on Learning Representations (2020).
\end{itemize}}

\newpage

\newperson{Reviewer 2}{R2}

\question{The authors extended their work entitled “Clinically-Inspired Multi-Agent Transformers for Disease Trajectory Forecasting from Multimodal Data” published in ISBI 2022. In this journal version, the authors further combined clinical non-imaging data with imaging data to forecast the severity
trajectory of the disease (AD and KOA).
This paper has several strengths:
\begin{itemize}
    \item This paper is well-written and implemented with well-designed figures, which benefits the reading.
    \item The evaluation metrics are sufficient and reasonable, especially in Table III.
    \item The idea of combing N unrolled visual feature vectors and clinical variables using Transformer (sequence-based) is simple and effective (at least from experiment results).
    \item The code is well-organized and the .readme file is clean and easy-to-follow.
\end{itemize}}

\answer{We thank the reviewer for rigorous feedback and in-depth comments. We will address the comments systematically.}

\question{The description of Transformer in Section III.B.1) is weak. The MSA operation is based on Q, K, V matrix, which should be described in detail. Whether Q and K are generated via the same linear projection function or other representation operation (convolution)?}

\answer{We learn query, key, and value parameters, denoted by $\bm{W}^Q_l, \bm{W}^K_l$, and $\bm{W}^V_l$ with $l=1,\dots,L$, respectively. Those parameters allow us to iteratively update the corresponding states $\bm{Q}_l, \bm{K}_l$, and $\bm{V}_l$. We improved the clarity of the MSA operator description starting line~\ref{ln:method_msa} of the revised manuscript.}

\question{As described in Fig. 4, M and N are determined by the dimension after the concatenation operation. I would like to see that how the ratio of M and N (M/N) will influence the subsequent results (down-sampling in N is suggested to conduct the ablation study.)}

\answer{In our settings, $N$ is determined by the depth of the CNN in the feature extraction module. Therefore, we cannot flexibly change $N$. Although we can decrease $N$ by using fewer convolutional blocks, such an action would change the receptive field of the CNN, which may result in unexpected behaviors. On the other hand, $M$ is associated with the number of non-imaging variables. Thus, decreasing $M$ leads to another non-trivial question of which variables we should drop. For those reasons, we fixed $N$ and $M$ depending on the nature of each dataset. As such, we had $N=64$ (with ResNet18 and input knee images with a pixel spacing of $0.5mm$) and $M=6$ for the knee data, and $N=131$ (with 4-convolutional layers of 3D-ShuffleNet2 and 3D PET scans with a voxel spacing of $1.5\times1.5\times1.5mm$) and $M=33$ for the brain data. We clarified the information at line~\ref{ln:exp_m_n} and supplement~\cref{tbl:oai_input,tbl:adni_input} of the revised manuscript.}
% \todo[inline]{You are asked to make an experiment here.}
\question{In section IV-A-2, the 2rd paragraph, ‘The raw FDG-PET scans were pre-processed by the dataset owner, and were then standardized to voxel dimensions of 160 × 160 × 160. To be in line with the OAI dataset.’ The voxel dimension is standardized to 160 × 160 × 160. From my understanding, the 3D registration or reshape operation in Numpy or Pytorch could both give the fixed dimension, which one is your operation, please make it specific.}

\answer{We used the $conform()$ function from the NiBabel library (\url{https://nipy.org/nibabel/}) to perform the voxel normalization. This is now mentioned in preprocessing line~\ref{ln:exp_vx_std} of the revised manuscript.}
% \todo[inline]{Mention size in millimeters in the text.}
\question{The competing baseline methods are weak, such as FCN, GRU, LSTM. There are many sequence-based Transformer algorithms that should be compared to illustrate the effectiveness of proposed method. The authors should compare at least two or three recent papers. For instance, literature [1] and [2] are suggested for comparison.
\begin{itemize}
    \item[] [1] Zhou, Haoyi, et al. "Informer: Beyond efficient transformer for long sequence time-series forecasting." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 35. No. 12. 2021.
    \item[] [2] Wu, Haixu, et al. "Autoformer: Decomposition transformers with auto-correlation for long-term series forecasting." Advances in Neural Information Processing Systems 34 (2021): 22419-22430.    
\end{itemize}}

\answer{Thanks to the reviewer for the suggestion, we have supplemented 3 more transformer-based baselines to the manuscript. Besides Informer and Autoformer, we also added Reformer [3] to the baseline list. To make the aforementioned baselines fit into the prognosis prediction setting, we kept most of the components of the pipeline standard except for the transformer-based encoder. Thus, the implementation of the new baselines is consistent with the MMTF reference with different transformer-based encoders. We present the results at Line~\ref{ln:exp_oai_former_results} in~\cref{sc:perf_comparisons}.
\begin{itemize}
    \item[] [3] Kitaev. N. et al. "Reformer: The Efficient Transformer." International Conference on Learning Representations (2020).
\end{itemize}}

\question{As CX and CM are concatenated, just like a feature fusion mechanism, whether the mix-up operation of CX and CM is superior to simple concatenation is suggested to illustrate}

\answer{Thank you for giving us a chance to express our finding of the concatenation of imaging and non-imaging embeddings. The concatenation makes dimensions of imaging and non-imaging embeddings flexible as they are not necessarily the same. The flexibility is needed because the clinical variables (e.g.\ age, sex, BMI) are much more semantically simple than imaging embeddings. In our experiments, we let $C_{X}=2C_{M}$. The idea the reviewer mentioned was implemented in the MMTF baseline~\cite{hu2021transformer}. According to~\cref{fig:oai_performances}, and~\cref{tbl:adni_performances}, our approach achieved superior performance compared to the baseline.}

\question{T-test should be conducted to prove the advantage of the  proposed method in Table III. Also, the caption should describe the meaning of underline and boldface in the table.}

\answer{To address the comment, we performed Wilcoxon signed-rank tests to verify significant differences between our method and each baseline, as the assumption for $t$-test do not hold for our data. Besides this, we added $*$ signs to~\cref{fig:oai_performances} and~\cref{tbl:adni_performances} to indicate the stastical tests' significance level (adjusted for multiple comparisons in the case of the OAI dataset). In addition, we improved the clarity of Table III's caption.}
% \todo[inline]{Let's see what the testing is. I am not sure about the t-test.}
\question{Fig. 8(a) is ambiguous, I don’t understand why the higher score of attention values appears out of the brain? I think the discussion of Figure 8(a) in the Conclusion section is weak. Do you take the average of the dataloader to show the attention map? Also, a binary brain template of the averaged brain template should take the inner-product to make sure that the attention scores are located in the brain.}

\answer{Thanks for your comments and suggestion. First, we refer the reviewer to our response to R1.6. Second, during the revision, we took a step back to give a critical look to our implementation of the attention maps. As suggested by the recent study of Nirthika \textit{et al.}~\cite{nirthika2022pooling}, we enhanced the noise robustness of the attention maps by applying average pooling instead of the max-pooling. Second, as the reviewer suggested, we enhanced the Conclusions section by supplementing the limitations of our framework at Line~\ref{ln:cons_limitations} of~\cref{sc:conclusions}, and provided more attention samples in~\cref{fig:adni_attn_examples}.
\begin{itemize}
    \item[] [4] R. Nirthika, S. Manivannan, A. Ramanan, and R. Wang, “Pooling in convolutional neural networks for medical image analysis: a survey and an empirical study,” Neural Computing and Applications, vol. 34, no. 7, 764 pp. 5321–5347, 2022.  
\end{itemize}}    
% \todo[inline]{This response needs more work. At the momemnt it contains only a few acceptance-leading bits of information for the reviewer. }
\question{The caption of Figure 2: The color of the arrow in the sub-figure is orange instead of red, please correct it.}

\answer{We have corrected this. Thanks for spotting!}

\question{On page 9/11 (3rd line under Fig. 6), our model achieved 1.3\%, 1.7\%, 1.9\%, 2.3\%, 0.7, 4.4\%. It seems that a ‘\%’ is missing after 0.7.}

\answer{Thanks! The typo has been corrected.}

\question{Fig. 6 should be revised. E.g. ‘OSFL’, ‘OSFM’ in the second line are suggested to be put in a proper position.}

\answer{The sub-captions were fixed as the reviewer has suggested.}

% \answer{We totally agree that it would be neater to make every single sub-caption fit well into one line. However, due to the width limit of each sub-figures on the second row of Fig. 6, and for the sake of completeness of the sub-captions, we are afraid that we have to accept the imperfection of the sug-figures (d) and (e).}
% \todo[inline]{Here we should please the reviewer and rework the figure.}
\question{In Section IV-B-1, the number of V100 GPUs is missing (the specific number could help readers understand the computational cost of your experiment). Also, please replace `NVidia’ by `Nvidia’.}

\answer{We clarified in the main text that each experimental setting was trained on a single V100 Nvidia GPU using a cluster of 320 GPUs. Each method was trained $5$ times with different random seeds. We performed $5$ and $10$-fold cross-validation strategies for the knee and brain data, respectively. Particularly, we had $7$ structural KOA grading sub-systems and systems. Thus, while we needed $5 (seeds)\times 5(folds)\times7(gradings)\times3(hours/exp.)=525$ GPU hours to produce results for each method on OAI data in~\cref{fig:oai_performances}, we used $5(seeds)\times10(folds)\times8(hours/exp.)=400$ GPU hours to generate results for each method on ADNI data in~\cref{tbl:adni_performances}. We have acknowledged CSC -- IT Center for Science of Finland -- in~\cref{sc:acknowledgement}.}

==> _responsesR2.tex <==
\onecolumn
\overview{Response Letter to Reviewers}
\newperson{Reviewer 1}{R1}

\question{The previous questions have been addressed. With the revised version, I only have the following minor comments:}

\answer{Thanks for the reviewer's efforts and insightful comments. We will address them in a point-by-point manner below.}

\question{What are the challenges of assuming $y_0$ and $m_0$ are not independent? Please elaborate more on the details.}

\answer{We believe that there are no challenges in assuming this. In fact, we consider that challenges come from assuming \textit{the opposite}, as we have done in the conference version of the paper. One of the goals of our current work was to expand the proposed method to a larger scope and make it more clinically applicable. 

To be more specific, we would like to refer to the works related directly to knee OA and Alzheimer's disease. For instance, it has been shown that using only clinical data, it is possible to predict early OA from non-imaging data [1]. Furthermore, adding clinical data to imaging may result in performance gains when it comes to the prediction of knee OA severity [2]. For the case of Alzheimer's disease, $y_0$ is actually defined from cognitive tests, and PET imaging data merely supports the longitudinal prediction of disease severity. Such a dependency can also be found in other diseases such as diabetes and COVID-19 [3,4].

Based on the aforementioned, 
% we conclude that the introduced modification to CLIMAT is justified, but 
we have added the needed clarifications at Lines~\ref{ln:version_cmp} and~\ref{ln:version_cmp2}, and improved the conclusion at Line~\ref{ln:conclusion_climat_cmp}.

\begin{itemize}
    \item[] [1] Liem, Y., Judge, A., Kirwan, J., Ourradi, K., Li, Y., \& Sharif, M. (2020). Multivariable logistic and linear regression models for identification of clinically useful biomarkers for osteoarthritis. Scientific Reports, 10(1), 11328.
    \item[] [2] Liu, L., Chang, J., Zhang, P., Ma, Q., Zhang, H., Sun, T., \& Qiao, H. (2023). A joint multi-modal learning method for early-stage knee osteoarthritis disease classification. Heliyon, 9(4).
   \item[] [3] Udler, M. S., McCarthy, M. I., Florez, J. C., \& Mahajan, A. (2019). Genetic risk scores for diabetes diagnosis and precision medicine. Endocrine reviews, 40(6), 1500-1520.   
   \item[] [4] Zhang, Z., Bi, Q., Fang, S., Wei, L., Wang, X., He, J., ... \& Zou, X. (2021). Insight into the practical performance of RT-PCR testing for SARS-CoV-2 using serological data: a cohort study. The Lancet Microbe, 2(2), e79-e87.
\end{itemize}
}
%\answer{Thanks for giving us a chance to emphasize the difference between the two versions of CLIMAT. We would like to point out that the dependence between $y_0$ and $m_0$ is not an assumption because a variety of evidence for the dependency has been found not only in knee osteoarthritis and Alzheimer's disease but also in other diseases. For instance, Liu~\etal~[1] provided empirical evidence for the benefit of combining imaging and non-imaging data for the KOA classification task. Bird~\etal~[2] showed a link between human genes and Alzheimer's disease. The study done by Li~\etal~[3] indicates that a blood test can detect the existence of amyloid-beta plaques in the brain, which is one of the characteristics of Alzheimer's disease. Furthermore, not limited to the two diseases studied in this work, non-imaging factors are predictive for other diseases. For instance, Udler~\etal~[4] and Cole~\etal~[5] showed the effectiveness of genetic data in diabetes diagnosis. Real-time reverse transcription–polymerase chain reaction (RT-PCR) tests are the most practical and effective tools for COVID-19 detections~[6,7]. \\
%To elaborate on the matter, we improved the clarification regarding the assumption of CLIMATv1 at Lines~\ref{ln:version_cmp} and~\ref{ln:version_cmp2}.
% \todo[inline]{Improve the discussion accordingly}
%\begin{itemize}
%    \item[] [1] Liu, L., Chang, J., Zhang, P., Ma, Q., Zhang, H., Sun, T., \& Qiao, H. (2023). A joint multi-modal learning method for early-stage knee osteoarthritis disease classification. Heliyon, 9(4).
%    \item[] [2] Bird, T. D. (2005). Genetic factors in Alzheimer's disease. New England Journal of Medicine, 352(9), 862-864.
%    \item[] [3] Li, Y., Schindler, S. E., Bollinger, J. G., Ovod, V., Mawuenyega, K. G., Weiner, M. W., ... \& Bateman, R. J. (2022). Validation of plasma amyloid-$\beta$ 42/40 for detecting Alzheimer disease amyloid plaques. Neurology, 98(7), e688-e699.
%    \item[] [4] Udler, M. S., McCarthy, M. I., Florez, J. C., \& Mahajan, A. (2019). Genetic risk scores for diabetes diagnosis and precision medicine. Endocrine reviews, 40(6), 1500-1520.
%    \item[] [5] Cole, J. B., \& Florez, J. C. (2020). Genetics of diabetes mellitus and diabetes complications. Nature reviews nephrology, 16(7), 377-390.
%    \item[] [6] Zhang, Z., Bi, Q., Fang, S., Wei, L., Wang, X., He, J., ... \& Zou, X. (2021). Insight into the practical performance of RT-PCR testing for SARS-CoV-2 using serological data: a cohort study. The Lancet Microbe, 2(2), e79-e87.
%    \item[] [7] Sule, W. F., \& Oluwayelu, D. O. (2020). Real-time RT-PCR for COVID-19 diagnosis: challenges and prospects. The Pan African Medical Journal, 35(Suppl 2).
%\end{itemize}}
% In general, the independence assumption between $y_0$ and $m_0$ can be stated as ``Non-imaging data such clinical, social, genetic factors are not predictive for the diagnosis of an arbitrary disease.'' We found such an assumption implied in the first version of CLIMAT was too strong and unrealistic. In other words, the dependency between the diagnosis task and non-imaging data is not an assumption

\question{The explanations in the last few lines in Sec III.B(3) are confusing. It seems the block P from the previous version can also make predictions. The importance or effects of using pooling to generate imaging representations is not clear.}

\answer{Thanks for pointing this out. We have made relevant changes at Line~\ref{ln:block_r} to improve the clarity of~\cref{sc:block_r}. Regarding the comments about the block P, we list the answers below:
\begin{itemize}
    \item In the first version of CLIMAT, this block \textit{does not} perform prediction of the current disease severity $y_0$ (see \cref{fig:climat_workflow}.a).
    \item For the second comment, we first would like to clarify that using average pooling in visual transformers is a common practice, and its benefits have been studied in [5-7]. 
\end{itemize}

While there can be many implementations of pooling, we conducted an ablation study on the matter, testing average pooling versus using just the first embedding from the block P. These results have been added to~\cref{tbl:hyperparam_selection}, and they show that utilizing average pooling leads to a performance gain of $1.1\%$ in BA, compared to using the first vector corresponding to the [CLS] embedding to make the diagnosis prediction $\hat{y}_0^R$. Furthermore, we added~\cref{sc:exp_image_rep} to present the experiments and their results.
\begin{itemize}
    \item[] [5] Pan, Z., Zhuang, B., Liu, J., He, H., \& Cai, J. (2021). Scalable vision transformers with hierarchical pooling. In Proceedings of the IEEE/cvf international conference on computer vision (pp. 377-386).
    \item[] [6] Park, N., \& Kim, S. (2022). How do vision transformers work?. arXiv preprint arXiv:2202.06709.
    \item[] [7] Chu, X., Tian, Z., Zhang, B., Wang, X., Wei, X., Xia, H., \& Shen, C. (2021). Conditional positional encodings for vision transformers. The Eleventh International Conference on Learning Representations (2023).
\end{itemize}}

\question{How to choose the value of inverse temperature to smoothen or sharpen?}

\answer{According to [8], the higher the temperature $\sigma^2$ is (equivalently, the lower the inverse temperature $\tau$ is), the more confident predictions the model tends to make, and vice versa. As calibration is of our interest, we aim to have the inverse temperature $\tau_t \leq 1$ (or temperature $\sigma_t^2 >= 1$). The reason is that low temperature in the softmax tends to avoid overconfident predictions~[11]. In the setting of CLUB loss, we have a set of $\{\tau\}_{t=0}^T$ (or $\{\sigma^2_t\}_{t=0}^T$) corresponding to $T+1$ prediction heads for the disease prognosis task. Values of $\sigma^2_t$'s are updated by backpropagating $\mathcal{L}_{\mathrm{prog}}$ in (12). Then, we applied Algorithm 1 to derive $\tau_t$'s.
\begin{itemize}
    \item[] [8] Hinton, G., Vinyals, O., \& Dean, J. (2015). Distilling the knowledge in a neural network. arXiv preprint arXiv:1503.02531. 
\end{itemize}}

\newpage

\newperson{Reviewer 3}{R3}

\question{The authors have addressed most of reviewers’ concerns in the previous round, however there are several issues for further improvement of the manuscript.}

\answer{We appreciate the reviewer's efforts in helping us to improve the paper. We address each of the reviewer's raised concerns below in a point-to-point manner.}

\question{For Fig. 4, there are indications of some numbers in the yellow box in (a), it is better to add the corresponding content in (b).}

\answer{Thanks! This has now been fixed.}%Thanks for the notice. Those indices are visible in the pdf file we uploaded. For some reason, they are only visible in individual PDF files as well as the PDF proof, but not in the HTML proof, which could be seen by reviewers. To address the issue, we use high-DPI images stead of PDF files for the workflows in~\cref{fig:climat_workflow}.}

\question{For Table I, there is no relevant introduction in the text. I wonder how to get the corresponding number of samples in Table 1 (such as using certain exclusion criteria, etc.).}

\answer{We have now supplemented proper introduction to~\cref{tbl:tasks_desc} at Line~\ref{ln:data_overview}. For clarification, we have added the details of subject selection in~\cref{fig:subject_selection}. Further data pre-processing steps have already been presented in~\cref{sc:oai_data,sc:adni_data}.}

% \begin{itemize}
%     \item[] [1] Lindner, C., Thiagarajah, S., Wilkinson, J. M., Wallis, G. A., Cootes, T. F., \& arcOGEN Consortium. (2013). Fully automatic segmentation of the proximal femur using random forest regression voting. IEEE transactions on medical imaging, 32(8), 1462-1472.
% \end{itemize}
% In the case of the OAI dataset, the subject count refers to the number of individual knees that were imaged at the baseline and successfully identified using the BoneFinder tool~[1]. As for the ADNI dataset, the count includes all participants who underwent FDG-PET scans at the baseline. 

\question{For Table IV, the corresponding prognosis task is based on which types of grading, the author should give more details.}

\answer{We improved the clarification of~\cref{tbl:hyperparam_selection}'s caption. Specifically, we clarified that the experiments were conducted using progression defined as changes in KL scores.}

\question{For Fig. 6, I can’t find where the ECEs are displayed.}

\answer{We supplemented the graphical plots for ECE comparisons in~\cref{fig:oai_cum_ece}.}

\question{For the response of Comment R1.3, the consistency regularization contributes to the model performance improvement when $\lambda$=0.5, but not for other values (i.e., 0.25, 0.75 and 1.0). The author should elaborate the role of consistency regularization in a more cautious manner. Moreover, I wonder if the model would benefit from the consistency regularization for the ECE metric and the ADNI cohort.}

\answer{Thanks for the comment. We agree with the reviewer and have conducted the experiments on other tasks and observed both performance and calibration gains as suggested by the reviewer. As such, we provided empirical results related to JSL, JSM, and AD in~\cref{tbl:effect_cons} and described the experiments at Line~\ref{ln:effect_cons2}. According to our findings, the consistency term tends to contribute to the performance gain of our method across the listed tasks, albeit with the trade-off of calibration.}

\question{For the response of Comment R2.6, It is unfair to simply compare concatenated and mix-up operation under different network architectures. The authors should provide the performance difference of only changing the feature fusion mechanism under the same network architecture. }

\answer{Thanks to the reviewer, we implemented the baseline as suggested. We present more empirical results on the multimodal combination approach in~\cref{sc:exp_channelwise_concat} and~\cref{tbl:ablation_emb_combination}. Over different forecasting tasks, our channel-wise concatenation approach results in high performance and tends to have lower ECEs.}

% that a more proper ablation study regarding the combination of imaging and non-imaging embeddings is needed. Specifically, the reference architecture was implemented to be similar to CLIMATv2 (i.e.\ including 3 transformer-based modules), except for the approach for combing imaging and non-imaging features. We had to employ a linear projection layer for non-imaging embeddings so that their feature dimension is consistent with imaging ones'. We then append projected non-imaging embeddings into imaging embeddings to form a sequence with a length of $N+M$. 

==> _revision_summary.tex <==
\onecolumn
\overview{[TMI-2022-1981] Revision Summary}

\begin{table}[htbp]
\renewcommand\thetable{}
\centering
\renewcommand{\arraystretch}{1.5}
\caption{}
\begin{tabular}{|r|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{\textbf{ID}} & \textbf{Section} & \textbf{Line/Reference} & \textbf{Changes} & \textbf{Related comments} \\ \hline
1 & Introduction & Caption of \cref{fig:progression_sample} & Corrected arrow color & R2.9 \\ \hline
2 & Methods & Line \ref{ln:method_msa} & Improve the clarity of MSA & R2.2 \\ \hline
3 & Methods & \cref{fig:climat_workflow} (a) & Fix missing '+' signs associated with blocks C and P & \\ \hline
4 & Experiments & Lines~\ref{ln:exp_pretrained_resnet} and~\ref{ln:exp_pretrained_3dshufflenet} & Improve the clarity of pretrained weights & R1.2 \\ \hline
5 & Experiments & Line \ref{ln:exp_m_n}, \cref{tbl:oai_input,tbl:adni_input} & Improve the clarity of input variables & R2.3 \\ \hline
6 & Experiments & Line \ref{ln:exp_vx_std} & Improve the clarity of voxel standardization & R2.4 \\ \hline
 % & Experiments & Line \ref{ln:formers_desc} & Describe more transformer-based baselines & R2.5 \\ \hline
7 & Experiments & Caption of \cref{tbl:adni_performances} & Improve the clarity of~\cref{tbl:adni_performances} (previously Table III) & R2.7 \\ \hline
8 & Experiments & Line \ref{ln:exp_missing_percent} & Fixed missing \% & R2.10 \\ \hline
9  & Experiments & Lines \ref{ln:metric_desc}, \ref{ln:adni_results},~\cref{fig:oai_performances} and \cref{tbl:adni_performances} & Describe metrics for evaluation and supplement statistical tests & R1.4 and R2.7 \\ \hline
10 & Experiments & Lines \ref{ln:formers_desc}, \ref{ln:exp_oai_former_results} & Describe Reformer, Informer, and Autoformer baselines & R1.7 and R2.5 \\ \hline
11 & Experiments & \cref{fig:oai_performances} and~\cref{tbl:adni_performances} & Supplement results of Reformer, Informer, and Autoformer & R1.7 and R2.5 \\ \hline
12 & Experiments & Line \ref{ln:exp_gpus} & Clarify about GPU usage & R2.12 \\ \hline
13 & Experiments & Line \ref{ln:adni_attn} and~\cref{fig:adni_interpretability} & Update attention maps on imaging data in~\cref{fig:adni_interpretability} & R1.6 and R2.8 \\ \hline
14 & Experiments & Line \ref{ln:adni_attn_result} & Improve clarity & \\ \hline
15 & Conclusions & Lines \ref{ln:attn_limitation_removed},~\ref{ln:cons_limitations} of~\cref{sc:conclusions} & Supplement limitations of our framework & R1.6 and R2.8 \\ \hline
16 & Conclusions & Line \ref{ln:conclusion_optimization} & Clarify the advantage of CLIMATv2 compared to CLIMATv1 & R1.5 \\ \hline
17 & Acknowledgement & \cref{sc:acknowledgement} & Add acknowledgement section & R2.12 \\ \hline
\end{tabular}
\end{table}



==> _revision_summaryR2.tex <==
\onecolumn
\overview{[TMI-2023-0758.R1] Revision Summary}

% \begin{table}[htbp]
% \renewcommand\thetable{}
% \centering
% \renewcommand{\arraystretch}{1.5}
% \caption{}
% \begin{tabular}{|r|l|l|l|c|}
% \hline
% \multicolumn{1}{|l|}{\textbf{ID}} & \textbf{Section} & \textbf{Line/Reference} & \textbf{Changes} & \textbf{Comments} \\ \hline
% 1 & Introduction & Line~\ref{ln:version_cmp} & \multirow{3}{*}{Improved the explanation of the assumption made in CLIMATv1} & \multirow{3}{*}{R1.2} \\ \cline{1-3}
% 2 & Methods & Line~\ref{ln:version_cmp2} & &  \\ \cline{1-3}
% 3 & Conclusions & Line~\ref{ln:conclusion_climat_cmp} & & \\ \hline
% 4 & Methods & Line~\ref{ln:block_r} & Improved the clarity of section III.B(3) & \multirow{2}{*}{R1.3} \\ \cline{1-4}
% 5 & Experiments & \cref{tbl:hyperparam_selection} ,~\cref{sc:exp_image_rep} & Supplemented ablation study on image representation for $\hat{y}_0^R$ prediction &  \\ \hline
% 6 & Methods & \cref{fig:climat_workflow} & Improved the visibility of indices & R3.2 \\ \hline
% 7 & Experiments & Caption of~\cref{tbl:tasks_desc},~\cref{fig:subject_selection}, and Line~\ref{ln:data_overview} & Improved details of subject selection and properly mentioned it in the text & \multirow{2}{*}{R3.3} \\ \cline{1-4}
% 8 & Experiments & Line~\ref{ln:syn_err1} & Fixed wrong reference & \\ \hline
% 9 & Experiments & Caption of~\cref{tbl:hyperparam_selection} & Improved the clarity of~\cref{tbl:hyperparam_selection}  & R3.4 \\ \hline
% 10 & Experiments & \cref{fig:oai_cum_ece} and Line~\ref{ln:oai_cum_ece} & Supplemented ECEs on the OAI dataset & R3.5 \\ \hline
% 11 & Experiments & \cref{tbl:effect_cons} and Line~\ref{ln:effect_cons} & Supplemented ablation study on the effect of the consistency term & R3.6 \\ \hline
% 12 & Experiments & \cref{tbl:ablation_emb_combination} and~\cref{sc:exp_channelwise_concat} & Supplemented ablation study on embedding combination approaches & R3.7 \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[htbp]
\renewcommand\thetable{}
\centering
\renewcommand{\arraystretch}{1.5}
\caption{}
\begin{tabular}{|r|c|l|l|l|}
    \hline
        \textbf{ID} & \textbf{Comments} & \textbf{Changes} & \textbf{Line/Reference} & \textbf{Section} \\ \hline
        1 & \multirow{3}{*}{R1.2} & \multirow{3}{*}{Improved the explanation of the assumption made in CLIMATv1} & Line~\ref{ln:version_cmp} & Introduction \\ \cline{1-1} \cline{4-5}
        2 &  &  & Line~\ref{ln:version_cmp2} & Methods \\ \cline{1-1} \cline{4-5}
        3 &  &  & Line~\ref{ln:conclusion_climat_cmp} & Conclusions \\ \hline
        4 & \multirow{2}{*}{R1.3} & Improved the clarity of section III.B(3) & Line~\ref{ln:block_r} & Methods \\ \cline{1-1} \cline{3-5}
        5 &  & Supplemented ablation study on image representation for $\hat{y}_0^R$ prediction & \cref{tbl:hyperparam_selection} ,~\cref{sc:exp_image_rep} & Experiments \\ \hline
        6 & R3.2 & Improved the visibility of indices & \cref{fig:climat_workflow} & Methods \\ \hline
        7 & \multirow{2}{*}{R3.3} & Improved details of subject selection and properly mentioned it in the text & \cref{fig:subject_selection}, and Line~\ref{ln:data_overview} & Experiments \\ \cline{1-1} \cline{3-5}
        8 &  & Fixed wrong reference & Line~\ref{ln:syn_err1} & Experiments \\ \hline
        9 & R3.4 & Improved the clarity of~\cref{tbl:hyperparam_selection} & Caption of~\cref{tbl:hyperparam_selection} & Experiments \\ \hline
        10 & R3.5 & Supplemented ECEs on the OAI dataset & \cref{fig:oai_cum_ece} and Line~\ref{ln:oai_cum_ece} & Experiments \\ \hline
        11 & R3.6 & Supplemented ablation study on the effect of the consistency term & \cref{tbl:effect_cons} and Line~\ref{ln:effect_cons} & Experiments \\ \hline
        12 & R3.7 & Supplemented ablation study on embedding combination approaches & \cref{tbl:ablation_emb_combination} and~\cref{sc:exp_channelwise_concat} & Experiments \\ \hline
        13 & & Move the paragraph to Line~\ref{ln:summary} & Line~\ref{ln:summary_prev} & Conclusions \\ \hline
        14 & & Minor changes & Caption of~\cref{tbl:tasks_desc}, Lines~\ref{ln:code} and \ref{ln:acknowledgement} & \\ \hline
    \end{tabular}
\end{table}

% sc:exp_channelwise_concat


==> bibtex/related_work.tex <==
\section{Related Work}

We observe that \cite{kendall2018multi} does not suppress well-classified samples and may result in negative losses (illustrated in \Cref{fig:mtl}).
